Proximal Gradient Algorithms: Applications in Signal Processing

Advances in numerical optimization have supported breakthroughs in several areas of signal processing. This paper focuses on the recent enhanced variants of the proximal gradient numerical optimization algorithm, which combine quasi-Newton methods with forward-adjoint oracles to tackle large-scale problems and reduce the computational burden of many applications. These proximal gradient algorithms are here described in an easy-to-understand way, illustrating how they are able to address a wide variety of problems arising in signal processing. A new high-level modeling language is presented which is used to demonstrate the versatility of the presented algorithms in a series of signal processing application examples such as sparse deconvolution, total variation denoising, audio de-clipping and others.

==> tables/convex_comp.tex <==
\glsunset{zerofpr}
\glsunset{ip}
\glsunset{scs}
\glsunset{fpg}

\begin{table*}[tb]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{center}
{ \small
\begin{tabularx}{0.9\textwidth}{c *{8}{Y}}
\toprule
                                                           &
  \multicolumn{5}{ c }{Using Matrices}                     &
  \multicolumn{3}{ c }{Matrix-Free   }                     \\

                                                           &
CVXOPT                                                   &
\gls{scs}                                                  &
\gls{pg}                                                   &
\gls{fpg}                                                  &
\gls{zerofpr}                                              &
\gls{pg}                                                   &
\gls{fpg}                                                  &
\gls{zerofpr}                                              \\
\cmidrule(lr){2-6} \cmidrule(l){7-9}
Sparse Deconvolution                                       &
%using mtx
%CVXOPT
54.3                                                      &
%SCS
11.0                                                      &
%PG
1.90                                                      &
%FPG
1.38                                                      &
%ZeroFPR
0.32                                                      &
%Mtx Free
%PG
0.45                                                      &
%FPG
0.31                                                      &
%ZeroFPR
0.07
                                                           \\
%\midrule
Line Spectral Estimation                                   &
%using mtx
%CVXOPT
71.3                                                     &
%SCS
35.2                                                     &
%PG
5.55                                                      &
%FPG
4.45                                                      &
%ZeroFPR
0.37                                                      &
%Mtx Free
%PG
0.93                                                      &
%FPG
0.73                                                      &
%ZeroFPR
0.10                                                      \\
\bottomrule
\end{tabularx}
}
\end{center}
\caption{
Table comparing the time (in seconds)
that different algorithm employ
to solve the convex problems appearing in
of \Cref{ex:sparse_deconv} and \Cref{ex:line_spectra}.
Both CVXOPT and \gls{scs} make use of
uses \cvxpy \cite{cvxpy}.
}
\label{tab:convex_comp}
\end{table*}

\glsreset{zerofpr}
\glsreset{ip}
\glsreset{scs}
\glsreset{fpg}


==> tables/scaled_lasso.tex <==

\begin{table*}[tb]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcolumntype{A}{>{\centering\arraybackslash\hsize=.4\hsize}X} 
\newcolumntype{B}{>{\centering\arraybackslash\hsize=.1\hsize}X}
\begin{center}
{ \small
\begin{tabularx}{\textwidth}{A B *{5}{ Y }}
\toprule
\midrule
                                                           & 
                                                           & 
  \multicolumn{2}{ c }{Conic Formulation}                  &
  \multicolumn{3}{ c }{Proximal Algorithms}                \\
\cmidrule(lr){3-4} \cmidrule(l){5-7}

&

&
ECOS     
&                                                           
SCS    
&                                                           
PG      
&                        
FPG     
& 
ZFPR 
\\
\midrule 
\multirow{2}{*}{ $ n = 10^3 $ } & $ t $ &  25.560 ms  &  78.110 ms  &  39.921 ms  &  12.560 ms  &  8.812 ms  \\ 
\cmidrule(lr){2-7}
                                & $ \epsilon $ & -148.3 & -81.1 & -88.2 & -98.1 & -97.9 \\ 
 \midrule 
\multirow{2}{*}{ $ n = 10^4 $ } & $ t $ &  1.481 s  &  2.394 s  &  3.774 s  &  137.852 ms  &  168.912 ms  \\ 
\cmidrule(lr){2-7}
                                & $ \epsilon $ & -118.7 & -59.1 & -63.1 & -65.6 & -63.6 \\ 
 \midrule 
\multirow{2}{*}{ $ n = 10^5 $ } & $ t $ &  2539.294 s  &  10.112 s  &  9.902 s  &  1.110 s  &  1.723 s  \\ 
\cmidrule(lr){2-7}
                                & $ \epsilon $ & -85.2 & -73.4 & -75.7 & -79.8 & -79.3 \\ 
 \midrule 
 \bottomrule
\end{tabularx}
}
\end{center}
\caption{
Table comparing the time $t$ 
and the error between the solution 
and the ground truth $\sig{\x}_{gt}$  
$\epsilon = 10 \log (\|\sig{\x}^{\star}-\sig{\x}_{gt} \|_2^2)$ 
of different algorithms.  
}
\label{tab:scaled_lasso}
\end{table*}


